Generalization Error Bounds with Probabilistic Guarantee for SGD in Nonconvex Optimization

The success of deep learning has led to a rising interest in the generalization property of the stochastic gradient descent (SGD) method, and stability is one popular approach to study it. Existing works based on stability have studied nonconvex loss functions, but only considered the generalization error of the SGD in expectation. In this paper, we establish various generalization error bounds with probabilistic guarantee for the SGD. Specifically, for both general nonconvex loss functions and gradient dominant loss functions, we characterize the on-average stability of the iterates generated by SGD in terms of the on-average variance of the stochastic gradients. Such characterization leads to improved bounds for the generalization error for SGD. We then study the regularized risk minimization problem with strongly convex regularizers, and obtain improved generalization error bounds for proximal SGD. With strongly convex regularizers, we further establish the generalization error bounds for nonconvex loss functions under proximal SGD with high-probability guarantee, i.e., exponential concentration in probability.

==> experiments.tex <==
%\section{Experimental Evaluation}\label{sec: exps}
%In this section, we provide experimental results on the generalization error of SGD.
%We perform two experiments: solving a logistic regression problem with the a9a data set \cite{Chang_2011} and training a three-layer ReLU neural network with the MNIST data set \cite{Lecun_1998}. For both experiments, we use a fixed initialization. We set the batch size to be 10 \% of the training sample size for the logistic regression and 160 for the neural network, and report the averaged results over multiple trials of the experiments. %(50 times for logistic regression and 10 times for neural network training).
%
%\textbf{Un-regularized optimization:}
%We first explore the generalization error and the training error when there is no regularizer in the objective function, and the results are shown in the left column of \Cref{fig: 1}. Note that the left y-axis corresponds to the generalization error curves and the right y-axis corresponds to the training error curves.
%
%It can be seen that the generalization error of SGD for logistic regression improves along the training epoches, and it increases only very slowly for neural network training. This is consistent with the theoretical result, which suggests that SGD can generalize well after multiple epoches. Also, it tends to support our theoretical finding that an amenable curvature of the problem helps to improve the generalization performance of SGD, as the logistic loss is a convex function with well curved geometry whereas the loss function of neural network is a highly nonconvex objective.
%
%%For logistic regression, one can see that a small batch size is preferred for SGD to have low training error and generalization error. While for the neural network,  the SGD generalizes better with a larger batch size, which, however, degrades the training error. Thus, a proper choice of batch size in training neural networks can have a balanced performance. These observations imply that the role of mini-batch size in our theoretical characterization may not be a dominant factor, and our bound can be pessimistic. We also note that for all experiments, the stepsize is chosen to be proportional to the batch size, and hence the observations may not be universal phenomena.
%
%
%
%\textbf{Regularized optimization:}
%We also explore the effect of regularization on the generalization error by adding the regularizer $\frac{\lambda}{2} \norm{\wb}^2$ to the objective functions. In particular, we apply the proximal SGD to solve the two problems. The right column of \Cref{fig: 1} shows the results. For both logistic regression and neural network training, it can be seen that the corresponding generalization errors improve (i.e., decrease) as the regularization weight increases. This agrees with our theoretical finding on the impact of regularization. On the other hand, the training performances for both problems degrade as the regularization weight increases beyond a certain threshold, which is reasonable because in such a case the optimization focuses too much on the regularizer and the obtained solution does not minimize the loss function well. Hence, there is a trade-off between the training performance and generalization performance in tuning the regularization parameter.































